Inducing Data Amplification Using Auxiliary Datasets in Adversarial Training

Several recent studies have shown that the use of extra in-distribution data can lead to a high level of adversarial robustness. However, there is no guarantee that it will always be possible to obtain sufficient extra data for a selected dataset. In this paper, we propose a biased multi-domain adversarial training (BiaMAT) method that induces training data amplification on a primary dataset using publicly available auxiliary datasets, without requiring the class distribution match between the primary and auxiliary datasets. The proposed method can achieve increased adversarial robustness on a primary dataset by leveraging auxiliary datasets via multi-domain learning. Specifically, data amplification on both robust and non-robust features can be accomplished through the application of BiaMAT as demonstrated through a theoretical and empirical analysis. Moreover, we demonstrate that while existing methods are vulnerable to negative transfer due to the distributional discrepancy between auxiliary and primary data, the proposed method enables neural networks to flexibly leverage diverse image datasets for adversarial training by successfully handling the domain discrepancy through the application of a confidence-based selection strategy. The pre-trained models and code are available at: \url{https://github.com/Saehyung-Lee/BiaMAT}.

==> Table/table_higher_than_thres_classes.tex <==
\begin{table*}[]
\centering
\caption{The mapping between CIFAR-10 superclasses and ImageNet classes for Table \ref{tab:table_confidence}.}
\label{tab:table_confidence_classes}
\small
%\resizebox{\columnwidth}{!} {
%\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}ll@{}}
\toprule
CIFAR-10 superclass & ImageNet classes \\ \midrule
Airplane & airliner, amphibian \\
&\\
Automobile & beach wagon, convertible, sports   car, ambulance, jeep, limousine, racer, cab, Model T \\
&\\
Bird & kite, white stork, ostrich, bustard, American egret, albatross, oystercatcher, \\
&red-breasted merganser,   dowitcher, bee eater, redshank, red-backed sandpiper, goldfinch, \\
&black stork,   crane, ruddy turnstone, bald eagle, partridge, magpie, black grouse, vulture,\\
&sulphur-crested cockatoo, junco, chickadee, American coot, spoonbill, quail, \\
&little blue heron, goose, indigo bunting, bulbul, pelican, brambling,   limpkin, coucal, robin,\\
&ptarmigan, house finch, European gallinule, ruffed   grouse, bittern, water ouzel, drake,\\
&peacock, jay, prairie chicken, jacamar,   black swan, hummingbird, African grey, hornbill, hen,\\
&great grey owl, cock,   king penguin, knot, toucan, lorikeet, flamingo, macaw \\
&\\
Cat & Persian cat, tabby, Egyptian cat,   Siamese cat, Angora, lynx, cheetah, tiger cat, lion, cougar, \\
&leopard, jaguar,   snow leopard, tiger \\
&\\
Deer & bison \\
&\\
Dog & Japanese spaniel, Maltese dog,   Pekinese, Shih-Tzu, Samoyed, Saint Bernard, Pomeranian,\\
&white wolf, Brabancon   griffon, Great Pyrenees, Newfoundland, miniature poodle, toy terrier,\\
&toy   poodle, chow, kit fox, Arctic fox, Mexican hairless, coyote, red wolf, red   fox, \\
&standard poodle, hyena, dhole, Eskimo dog, Great Dane, Rhodesian   ridgeback, keeshond, \\
&Pembroke, Chihuahua, bull mastiff, dingo, Cardigan,   timber wolf, boxer, basenji, grey fox,\\
&pug, African hunting dog, Leonberg,   dalmatian \\
&\\
Frog & tailed frog, tree frog, bullfrog \\
&\\
Horse & sorrel \\
&\\
Ship & yawl, speedboat, fireboat,   lifeboat, canoe, gondola \\
&\\
Truck & pickup, police van, trailer truck,   minivan, moving van, tow truck, fire engine, garbage truck, tractor \\ \bottomrule
\end{tabular}
%}
\end{table*}
